Variation Enhanced Attacks Against RRAM-based Neuromorphic Computing System

The RRAM-based neuromorphic computing system has amassed explosive interests for its superior data processing capability and energy efficiency than traditional architectures, and thus being widely used in many data-centric applications. The reliability and security issues of the NCS therefore become an essential problem. In this paper, we systematically investigated the adversarial threats to the RRAM-based NCS and observed that the RRAM hardware feature can be leveraged to strengthen the attack effect, which has not been granted sufficient attention by previous algorithmic attack methods. Thus, we proposed two types of hardware-aware attack methods with respect to different attack scenarios and objectives. The first is adversarial attack, VADER, which perturbs the input samples to mislead the prediction of neural networks. The second is fault injection attack, EFI, which perturbs the network parameter space such that a specified sample will be classified to a target label, while maintaining the prediction accuracy on other samples. Both attack methods leverage the RRAM properties to improve the performance compared with the conventional attack methods. Experimental results show that our hardware-aware attack methods can achieve nearly 100% attack success rate with extremely low operational cost, while maintaining the attack stealthiness.

==> coverletter.tex <==


\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/coverletter.pdf}
  \vspace{0.5\baselineskip}
\end{figure*}
% \begin{figure*}

% \noindent Dear Editors:

% % \\ \hspace*{\fill} \\

% This work entitled “Variation Enhanced Attacks Against RRAM-based Neuromorphic Computing System” is an extended version of [Lv et al. 2021] which was published at 2021 26th Asia and South Pacific Design Automation Conference (ASP-DAC), entitled “VADER: Leveraging the Natural Variation of Hardware to Enhance Adversarial Attack”. In the conference version, an enhanced adversarial attack for the RRAM-based devices was proposed, which leverages the intrisic RRAM variations to achieve better effectiveness and stealthiness compared with the previous algorithmic approaches. In comparison with the conference version, we have made substantial revisions and additions. Additional materials provided in this new manuscript compared to [Lv et al. 2021] are summarized below:


% 1. We systematically rewrite the whole manuscript compared to [Lv et al. 2021]. We provided the new version of figures and tables. 


% 2. We propose a new fault injection attack, EFI, on the RRAM-based neuromorphic computing system. In this method, we leverage the intrinsic RRAM variations to reduce the required modifications on the parameter space for a successful attack, considering that the fault injection operation is engineer expensive.
% The injected faults can incorporate with the existing RRAM variations to manuplate the network prediction for a specified sample to the desired result at ease, while maintaining accuracy on other samples.
% To be clear, we provided exhaustive descriptions and figures in Section V C (2) to demonstrate the effectiveness, efficiency and stealthiness of EFI. 


% 3. we extend the effectiveness evaluation for VADER. We evaluate VADER on different RRAM devices with different variation distributions to demonstrate the performance consistency.


% 4. We provided the efficiency and stealthiness evaluation of EFI, which is reported in Section V C (2).
% In the evaluation, we make a comparison with other SOTA fault injection attacks for neural networks to assess the improvement on efficiency and stealthiness and the benefit of our hardware aware philosophy.


% 5. In the experiment part, we further provide the analysis of the characteristic VADER and EFI, and discuss the feasible apporaches to resist the two variation oriented attack methods. 


% All the above extensions make this manuscript offer complete solutions for misleading the RRAM-based neuromorphic computing system with respect to different attack scenarios and objectives. We believe our new manuscript includes a significant new portion of contributions with respect to our ASP-DAC paper (e.g., \textgreat 30\%) and meets the requirement of TCAD. 
% We deeply appreciate your consideration of our manuscript, and we look forward to receiving comments from the reviewers. If you have any queries, please don’t hesitate to contact me.

% Sincerely,

% Hao Lv

% E-mail:lvhao21b@ict.ac.cn


% \end{figure*}
% \newpage
